Comparative Study of Virtual Machines and Containers for DevOps Developers

This paper presents a comparative study of virtual machines (VMs) and containers for DevOps developers. The study explores the benefits and drawbacks of each technology in terms of their functionality, performance, security, and resource utilization. The paper examines the underlying architecture of VMs and containers, and how they differ from each other. The study includes a series of experiments that compare the performance and resource utilization of VMs and containers in different scenarios. The experiments evaluate factors such as startup time, memory usage, disk I/O, network latency, scalability, and administrative overhead. Finally, the paper provides recommendations for DevOps developers on which technology to choose based on their specific requirements and use cases. Overall, the study aims to provide a comprehensive understanding of the strengths and limitations of VMs and containers, helping developers to make informed decisions when choosing between them.

==> IEEE Comparative Study of VMs and Containers-3/bibliography.tex <==
\bibliographystyle{IEEEtran}

@ARTICLE{bib1,
  author={Bernstein, David},
  journal={IEEE Cloud Computing}, 
  title={Containers and Cloud: From LXC to Docker to Kubernetes}, 
  year={2014},
  volume={1},
  number={3},
  pages={81-84},
  doi={10.1109/MCC.2014.51}}

@INPROCEEDINGS{bib2,
  author={Kang, Hui and Le, Michael and Tao, Shu},
  booktitle={2016 IEEE International Conference on Cloud Engineering (IC2E)}, 
  title={Container and Microservice Driven Design for Cloud Infrastructure DevOps}, 
  year={2016},
  volume={},
  number={},
  pages={202-211},
  doi={10.1109/IC2E.2016.26}}

@article{bib3,
title = {A summary of virtualization techniques},
journal = {Procedia Technology},
volume = {3},
pages = {267-272},
year = {2012},
note = {The 2012 Iberoamerican Conference on Electronics Engineering and Computer Science},
issn = {2212-0173},
doi = {https://doi.org/10.1016/j.protcy.2012.03.029},
url = {https://www.sciencedirect.com/science/article/pii/S2212017312002587},
author = {Fernando Rodríguez-Haro and Felix Freitag and Leandro Navarro and Efraín Hernánchez-sánchez and Nicandro Farías-Mendoza and Juan Antonio Guerrero-Ibáñez and Apolinar González-Potes}
}

@article{bib4,
title = {Cloud computing — The business perspective},
journal = {Decision Support Systems},
volume = {51},
number = {1},
pages = {176-189},
year = {2011},
issn = {0167-9236},
doi = {https://doi.org/10.1016/j.dss.2010.12.006},
url = {https://www.sciencedirect.com/science/article/pii/S0167923610002393},
author = {Sean Marston and Zhi Li and Subhajyoti Bandyopadhyay and Juheng Zhang and Anand Ghalsasi}
}

@article{bib5,
  title={Hypervisor: A survey on concepts and taxonomy},
  author={Desai, Ankita and Oza, Rachana and Sharma, Pratik and Patel, Bhautik},
  journal={International Journal of Innovative Technology and Exploring Engineering},
  volume={2},
  number={3},
  pages={222--225},
  year={2013},
  publisher={Citeseer}
}

@ARTICLE{bib6,
  author={Vaughan-nichols, Stephen J.},
  journal={Computer}, 
  title={New Approach to Virtualization Is a Lightweight}, 
  year={2006},
  volume={39},
  number={11},
  pages={12-14},
  doi={10.1109/MC.2006.393}}

@ARTICLE{bib7,
  author={Ebert, Christof and Gallardo, Gorka and Hernantes, Josune and Serrano, Nicolas},
  journal={IEEE Software}, 
  title={DevOps}, 
  year={2016},
  volume={33},
  number={3},
  pages={94-100},
  doi={10.1109/MS.2016.68}}

@ARTICLE{bib8,
  author={Zhu, Liming and Bass, Len and Champlin-Scharff, George},
  journal={IEEE Software}, 
  title={DevOps and Its Practices}, 
  year={2016},
  volume={33},
  number={3},
  pages={32-34},
  doi={10.1109/MS.2016.81}}

@INPROCEEDINGS{bib9,
  author={Felter, Wes and Ferreira, Alexandre and Rajamony, Ram and Rubio, Juan},
  booktitle={2015 IEEE International Symposium on Performance Analysis of Systems and Software (ISPASS)}, 
  title={An updated performance comparison of virtual machines and Linux containers}, 
  year={2015},
  volume={},
  number={},
  pages={171-172},
  doi={10.1109/ISPASS.2015.7095802}}

@misc{bib10,
  author = {O'Reilly Media},
  title = {Five Security Concerns When Using Docker},
  howpublished = {\url{https://www.oreilly.com/ideas/five-security-concerns-when-using-docker}},
  year = {2015},
  month = {June}
}

@article{bib11,
  title={The LINPACK benchmark: past, present and future},
  author={Dongarra, Jack J and Luszczek, Piotr and Petitet, Antoine},
  journal={Concurrency and Computation: practice and experience},
  volume={15},
  number={9},
  pages={803--820},
  year={2003},
  publisher={Wiley Online Library}
}

@inproceedings{bib12,
  title={Checkpoint/restart of virtual machines based on Xen},
  author={Vallee, Geoffroy and Naughton, Thomas and Ong, Hong and Scott, Stephen L},
  booktitle={Proceedings of the High Availability and Performace Computing Workshop (HAPCW 2006), Santa Fe, New Mexico, USA},
  year={2006}
}

==> bibliography.tex <==
\bibliographystyle{IEEEtran}

@ARTICLE{bib1,
  author={Bernstein, David},
  journal={IEEE Cloud Computing}, 
  title={Containers and Cloud: From LXC to Docker to Kubernetes}, 
  year={2014},
  volume={1},
  number={3},
  pages={81-84},
  doi={10.1109/MCC.2014.51}}

@INPROCEEDINGS{bib2,
  author={Kang, Hui and Le, Michael and Tao, Shu},
  booktitle={2016 IEEE International Conference on Cloud Engineering (IC2E)}, 
  title={Container and Microservice Driven Design for Cloud Infrastructure DevOps}, 
  year={2016},
  volume={},
  number={},
  pages={202-211},
  doi={10.1109/IC2E.2016.26}}

@article{bib3,
title = {A summary of virtualization techniques},
journal = {Procedia Technology},
volume = {3},
pages = {267-272},
year = {2012},
note = {The 2012 Iberoamerican Conference on Electronics Engineering and Computer Science},
issn = {2212-0173},
doi = {https://doi.org/10.1016/j.protcy.2012.03.029},
url = {https://www.sciencedirect.com/science/article/pii/S2212017312002587},
author = {Fernando Rodríguez-Haro and Felix Freitag and Leandro Navarro and Efraín Hernánchez-sánchez and Nicandro Farías-Mendoza and Juan Antonio Guerrero-Ibáñez and Apolinar González-Potes}
}

@article{bib4,
title = {Cloud computing — The business perspective},
journal = {Decision Support Systems},
volume = {51},
number = {1},
pages = {176-189},
year = {2011},
issn = {0167-9236},
doi = {https://doi.org/10.1016/j.dss.2010.12.006},
url = {https://www.sciencedirect.com/science/article/pii/S0167923610002393},
author = {Sean Marston and Zhi Li and Subhajyoti Bandyopadhyay and Juheng Zhang and Anand Ghalsasi}
}

@article{bib5,
  title={Hypervisor: A survey on concepts and taxonomy},
  author={Desai, Ankita and Oza, Rachana and Sharma, Pratik and Patel, Bhautik},
  journal={International Journal of Innovative Technology and Exploring Engineering},
  volume={2},
  number={3},
  pages={222--225},
  year={2013},
  publisher={Citeseer}
}

@ARTICLE{bib6,
  author={Vaughan-nichols, Stephen J.},
  journal={Computer}, 
  title={New Approach to Virtualization Is a Lightweight}, 
  year={2006},
  volume={39},
  number={11},
  pages={12-14},
  doi={10.1109/MC.2006.393}}

@ARTICLE{bib7,
  author={Ebert, Christof and Gallardo, Gorka and Hernantes, Josune and Serrano, Nicolas},
  journal={IEEE Software}, 
  title={DevOps}, 
  year={2016},
  volume={33},
  number={3},
  pages={94-100},
  doi={10.1109/MS.2016.68}}

@ARTICLE{bib8,
  author={Zhu, Liming and Bass, Len and Champlin-Scharff, George},
  journal={IEEE Software}, 
  title={DevOps and Its Practices}, 
  year={2016},
  volume={33},
  number={3},
  pages={32-34},
  doi={10.1109/MS.2016.81}}

@INPROCEEDINGS{bib9,
  author={Felter, Wes and Ferreira, Alexandre and Rajamony, Ram and Rubio, Juan},
  booktitle={2015 IEEE International Symposium on Performance Analysis of Systems and Software (ISPASS)}, 
  title={An updated performance comparison of virtual machines and Linux containers}, 
  year={2015},
  volume={},
  number={},
  pages={171-172},
  doi={10.1109/ISPASS.2015.7095802}}

@misc{bib10,
  author = {O'Reilly Media},
  title = {Five Security Concerns When Using Docker},
  howpublished = {\url{https://www.oreilly.com/ideas/five-security-concerns-when-using-docker}},
  year = {2015},
  month = {June}
}

@article{bib11,
  title={The LINPACK benchmark: past, present and future},
  author={Dongarra, Jack J and Luszczek, Piotr and Petitet, Antoine},
  journal={Concurrency and Computation: practice and experience},
  volume={15},
  number={9},
  pages={803--820},
  year={2003},
  publisher={Wiley Online Library}
}

@inproceedings{bib12,
  title={Checkpoint/restart of virtual machines based on Xen},
  author={Vallee, Geoffroy and Naughton, Thomas and Ong, Hong and Scott, Stephen L},
  booktitle={Proceedings of the High Availability and Performace Computing Workshop (HAPCW 2006), Santa Fe, New Mexico, USA},
  year={2006}
}
